Approximation Methods for Simulation and Equivalence Checking of Noisy Quantum Circuits

In the current NISQ (Noisy Intermediate-Scale Quantum) era, simulating and verifying noisy quantum circuits is crucial but faces challenges such as quantum state explosion and complex noise representations, constraining simulation and equivalence checking to circuits with a limited number of qubits. This paper introduces an approximation algorithm for simulating and assessing the equivalence of noisy quantum circuits, specifically designed to improve scalability under low-noise conditions. The approach utilizes a novel tensor network diagram combined with singular value decomposition to approximate the tensors of quantum noises. The implementation is based on Google's TensorNetwork Python package for contraction. Experimental results on realistic quantum circuits with realistic hardware noise models indicate that our algorithm can simulate and check the equivalence of QAOA (Quantum Approximate Optimization Algorithm) circuits with around 200 qubits and 20 noise operators, outperforming state-of-the-art approaches in scalability and speed.

==> figures/cucz.tex <==
\[
\begin{array}{c}\begin{aligned}
		\Qcircuit @C=1.5em @R=1.5em {
			& \ctrl{1} & \qw\\
			&\gate{U} & \qw}
	\end{aligned}
	=\left(\begin{matrix}1&0&0&0\\
		0&1&0&0\\
		0 & 0 & u_{00} & u_{01} \\
		0 & 0 & u_{10} & u_{11}
	\end{matrix}\right)\\
\end{array}
\begin{array}{c}\begin{aligned}
		\Qcircuit @C=1em @R=1em {
			& \ctrl{1} & \qw \\
			& \ctrl{-1} & \qw}
	\end{aligned}
	=\left(\begin{matrix}1&0&0&0\\
		0&1&0&0\\
		0&0&1&0\\
		0&0&0&-1
	\end{matrix}\right)\\
	% \text{Circuit representations for CU and CZ gates}
\end{array}
\]

==> figures/decomposition_a.tex <==
\begin{align*}
	&\begin{aligned}
		\Qcircuit @C=1em @R=1em{
			& \ustick{1} \qw  & \multigate{1}{M_\e}   & \ustick{3} \qw\\
			& \ustick{2} \qw  & \ghost{M_\e}          & \ustick{4} \qw\\}
	\end{aligned}
	\xRightarrow{\text{Permutation}} \begin{aligned}
		\Qcircuit @C=1em @R=1em{
			& \multigate{1}{\widetilde{M_\e}} & \qw \\
			& \ghost{\widetilde{M_\e}} & \qw \\}
	\end{aligned}
	= \begin{aligned}
		\Qcircuit @C=1em @R=1em{
			& \ustick{1} \qw &\multigate{1}{M_\e} & \ustick{2} \qw\\
			& \ustick{3} \qw &\ghost{M_\e} & \ustick{4} \qw}
	\end{aligned}
\end{align*}

==> figures/decomposition_c.tex <==
\begin{align*}
	\sum\limits_{i=0}^3\raisebox{-0.5\height}{%
		\begin{tikzpicture}
			% Define the nodes for the quantum gates and labels
			\node[draw,rectangle,minimum width=0.5cm, minimum height = 1cm] (u) at (0,1) {$\widetilde{U}_{i}$};
			\node[draw,rectangle,minimum width=0.5cm, minimum height = 1cm] (v) at (0.8,1) {$\widetilde{V}_{i}$};
			% Draw the lines (wires) extending out from the gates
			\draw (u.west) ++ (0, 0.2) -- ++(-0.1,0);
			\draw (u.west) ++ (0, -0.2) -- ++(-0.1,0);
			\draw (v.east) ++ (0, 0.2) -- ++(0.1,0);
			\draw (v.east) ++ (0, -0.2) -- ++(0.1,0);
		\end{tikzpicture}
	}
	\xRightarrow{\text{Permutation}} 
	\sum\limits_{i=0}^3\begin{aligned}
		\Qcircuit @C=1em @R=1em{
			& \gate{U_i} & \qw \\
			& \gate{V_i} & \qw \\}
	\end{aligned}
	=\begin{aligned}
		\Qcircuit @C=1em @R=1em{
			& \multigate{1}{M_\e} & \qw \\
			& \ghost{M_\e} & \qw \\}
	\end{aligned}
\end{align*}

==> figures/double_example.tex <==
\begin{align*}
	\begin{array}{c}
		\Qcircuit @C=0.5em @R=0.5em @!R {
			\lstick{\tikzdiagram{\node[fill=white,tensor,overlay,anchor=base,xshift=2pt] {$\bra{0}$};}} & \gate{\mathrm{R_Y}} & \gate{\mathrm{R_Z}} & \ctrl{1}  & \qw & \ctrl{1} & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})} & \gate{\ket{0}} \\
			\lstick{\tikzdiagram{\node[fill=white,tensor,overlay,anchor=base,xshift=2pt] {$\bra{0}$};}} & \gate{\mathrm{R_Y}} & \gate{\mathrm{R_Z}} & \control\qw & \gate{\tikz{\node[inner sep=0] (a){$\e_D$};}} \qwx[2] & \control\qw & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})} & \gate{\ket{0}} \\
			\lstick{\tikzdiagram{\node[fill=white,tensor,overlay,anchor=base,xshift=2pt] {$\bra{0}$};}} & \gate{\mathrm{R_Y}^*} & \gate{\mathrm{R_Z}^*} & \ctrl{1} &  \qw & \ctrl{1} & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})^*} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})^*} & \gate{\ket{0}} \\
			\lstick{\tikzdiagram{\node[fill=white,tensor,overlay,anchor=base,xshift=2pt] {$\bra{0}$};}}  & \gate{\mathrm{R_Y}}& \gate{\mathrm{R_Z}} & \control\qw & \gate{\tikz{\node[inner sep=0] (b){$\e_D^*$};}}& \control\qw & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})^*} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})^*} & \gate{\ket{0}}
			% \gategroup{2}{5}{2}{5}{.75em}{.}
			% \gategroup{4}{5}{4}{5}{.75em}{.}
		}
		% \\\text{2-qubit faulty QAOA circuit with the output state $\ket{ v }$ unknown, \\ the tensor network of $U \ket{0}$ is appended to the right side and the $R_x$ gates have been cancelled out.\\(Rotation angles in the left side is same with the previous figure and omitted) }
	\end{array}
\end{align*}

==> figures/double_example_eqc.tex <==
\begin{align*}
	\begin{array}{c}
		\Qcircuit @C=0.5em @R=0.5em @!R {
			\lstick{\tikz[remember picture] \node (start1) {};} & \gate{\mathrm{R_Y}} & \gate{\mathrm{R_Z}} & \ctrl{1}  & \qw & \ctrl{1} & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})} & \qw & \tikz[remember picture] \node (end1) {}; \\
			\lstick{\tikz[remember picture] \node (start2) {};} & \gate{\mathrm{R_Y}} & \gate{\mathrm{R_Z}} & \control\qw & \gate{\tikz{\node[inner sep=0] (a){$\e_D$};}} \qwx[2] & \control\qw & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})} & \qw & \tikz[remember picture] \node (end2) {}; \\
			\lstick{\tikz[remember picture] \node (start3) {};} & \gate{\mathrm{R_Y}^*} & \gate{\mathrm{R_Z}^*} & \ctrl{1} &  \qw & \ctrl{1} & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})^*} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})^*} & \qw & \tikz[remember picture] \node (end3) {}; \\
			\lstick{\tikz[remember picture] \node (start4) {};} & \gate{\mathrm{R_Y}}& \gate{\mathrm{R_Z}} & \control\qw & \gate{\tikz{\node[inner sep=0] (b){$\e_D^*$};}}& \control\qw & \gate{\mathrm{R_Z}\,(\mathrm{\frac{-\pi}{2}})^*} & \gate{\mathrm{R_Y}\,(\mathrm{\frac{\pi}{2}})^*} & \qw & \tikz[remember picture] \node (end4) {};
		}
	\end{array}
\end{align*}

==> figures/mat_rep_tn.tex <==
\begin{align*}
	M_{\e}&=\sum_{k\in\k}E_{k}\otimes E_{k}^*=\begin{aligned}
		\Qcircuit @C=1em @R=1em{
			&\gate{E_k} & \qw\\
			&\gate{E_k*} \qwx &\qw}\end{aligned} \\
	M_{\u}&=U\otimes U^*=\begin{aligned}
		\Qcircuit @C=1em @R=1em{
			&\gate{U} & \qw\\
			&\gate{U^*} &\qw}\end{aligned}
\end{align*}

==> figures/workflow.tex <==
\tikzset{module/.append style={top color=\col,bottom color=\col}}
\tikzset{every shadow/.style={fill=none,shadow scale=0}}
\smartdiagramset{
	back arrow disabled=true,
	set color list={red!22,cyan!22,blue!22,green!22},
	additions={
		additional item offset=0.85cm,
		additional item border color=black,
		additional connections disabled=false,
	}
}
\smartdiagramadd[flow diagram:horizontal]{
	Circuit under Test, Fault Simulator, Fault Effect, DFT/ATPG
}{
	below of module2/Fault Model, above of module2/Test Patterns
}

==> tables/eqc_compare.tex <==
\begin{table*}[]
	\centering
	\caption{\textsc{OUR ALGORITHM VS. ACCURATE METHODS (EQUIVALENCE CHECKING)}}
	% Please add the following required packages to your document preamble:
	% \usepackage{multirow}
	\begin{tblr}{
			cells = {c},
			cell{1}{1} = {r=2}{},
			cell{1}{2} = {r=2}{},
			cell{1}{3} = {r=2}{},
			cell{1}{4} = {r=2}{},
			cell{1}{5} = {c=3}{},
			cell{3}{1} = {r=2}{},
			cell{5}{1} = {r=2}{},
			cell{7}{1} = {r=4}{},
			cell{11}{1} = {r=3}{},
			cell{14}{1} = {r=8}{},
			vlines,
			hline{1,3,5,7,11,14,22} = {-}{},
			hline{2} = {5-7}{},
			hline{4,6,8-10,12-13,15-21} = {2-7}{},
		}
		Type      & Qubits & Gates & Depth & \#Noise = 20 &         &         \\
		&        &       &       & TDD          & TN      & Ours    \\
		BV        & 500    & 1499  & 502   & 17.53        & 22.28   & 19.94   \\
		& 10000  & 29999 & 10002 & 108.94       & 131.84  & 118.39  \\
		QFT       & 10     & 235   & 69    & 164.83       & 23.74   & 12.48   \\
		& 35     & 3010  & 271   & TO           & 2490.68 & 824.39  \\
		HF-VQE    & 6      & 155   & 72    & 4.84         & 3.06    & 3.78    \\
		& 8      & 308   & 124   & 10.48        & 2.15    & 2.64    \\
		& 10     & 461   & 142   & 4.22         & 2.84    & 2.34    \\
		& 12     & 690   & 194   & 3.85         & 1.5     & 1.03    \\
		QAOA      & 121    & 3322  & 42    & TO           & 1232.21 & 2709.46 \\
		& 169    & 4706  & 42    & TO           & 5033.26 & 4897.58 \\
		& 196    & 5488  & 42    & TO           & MO      & 8496.4  \\
		Supermacy & 16     & 115   & 11    & 118.38       & 18.9    & 6.23    \\
		& 16     & 209   & 21    & TO           & 152.46  & 9.03    \\
		& 16     & 299   & 31    & TO           & MO      & 30.85   \\
		& 16     & 394   & 41    & TO           & MO      & 78.4    \\
		& 20     & 145   & 11    & 193.64       & 130.57  & 29.13   \\
		& 20     & 261   & 21    & TO           & MO      & 18.64   \\
		& 20     & 378   & 31    & TO           & MO      & 1311.51 \\
		& 36     & 264   & 11    & TO           & MO      & 5069.82 
	\end{tblr}
	\label{table:AEC_compare}
\end{table*}

==> tables/eqc_level.tex <==
\begin{table}[htbp]
	\centering
	\caption{\textsc{Accuracy for Different Approximation Levels (Equivalence Checking)}}
	\begin{tabular}{|l|l|l|l|}
		\hline
		Level & Time (s) & Result   & Error    \\ \hline
		0     & 1.74     & 0.967819 & 1.33E-02 \\ \hline
		1     & 39.48    & 0.979301 & 8.86E-05 \\ \hline
		2     & 183.96   & 0.979386 & 3.60E-06 \\ \hline
		3     & 3029.5   & 0.979386 & 3.28E-06 \\ \hline
	\end{tabular}
	\label{table:AEC_approximate_level}
\end{table}

==> tables/mps_compare.tex <==
\begin{table*}[]
	\centering
	\caption{\textsc{Our Algorithm v.s. MPO-based Methods}}
	\begin{tblr}{
			cells = {c},
			cell{1}{1} = {r=3}{},
			cell{1}{2} = {r=3}{},
			cell{1}{3} = {r=3}{},
			cell{1}{4} = {r=3}{},
			cell{1}{5} = {c=5}{},
			cell{1}{10} = {c=5}{},
			cell{2}{5} = {r=2}{},
			cell{2}{6} = {c=2}{},
			cell{2}{8} = {c=2}{},
			cell{2}{10} = {r=2}{},
			cell{2}{11} = {c=2}{},
			cell{2}{13} = {c=2}{},
			cell{4}{1} = {r=3}{},
			cell{7}{1} = {r=8}{},
			vlines,
			hline{1,4,7,15} = {-}{},
			hline{2} = {5-14}{},
			hline{3} = {6-9,11-14}{},
			hline{5-6,8-14} = {2-14}{},
		}
		Type      & Qubits & Gates & Depth & Simulation &         &         &           &          & Equivalence Checking &         &         &           &          \\
		&        &       &       & Bond       & Time    &         & Precision &          & Bond                 & Time    &         & Precision &          \\
		&        &       &       &            & MPO     & Ours    & MPO       & Ours     &                      & MPO     & Ours    & MPO       & Ours     \\
		QAOA      & 121    & 3322  & 42    & 400        & 803.38  & 408.05  & 8.94E-05  & 1.28E-05 & 800                  & 1501.85 & 2709.46 & 7.59E-05  & 1.06E-05 \\
		& 169    & 4706  & 42    & 400        & 2604.05 & 2749.51 & 2.89E-05  & 4.82E-05 & 600                  & 4761.68 & 4897.58 & 2.41E-05  & 5.38E-05 \\
		& 196    & 5488  & 42    & 400        & 3392.5  & 4839.57 & 1.47E-04  & 1.49E-05 & 600                  & 6406.01 & 8496.4  & 1.02E-05  & 1.27E-05 \\
		Supermacy & 16     & 115   & 11    & 200        & 18.91   & 12.84   & 1.30E-02  & 2.87E-04 & 400                  & 34.17   & 6.23    & 1.29E-03  & 3.16E-04 \\
		& 16     & 209   & 21    & 200        & 36.59   & 28.88   & 9.00E-03  & 3.29E-04 & 400                  & 69.08   & 9.03    & 7.32E-04  & 3.25E-04 \\
		& 16     & 299   & 31    & 200        & 58.85   & 49.61   & 2.30E-02  & 7.39E-04 & 400                  & 108.89  & 30.85   & 2.29E-03  & 7.63E-04 \\
		& 16     & 394   & 41    & 200        & 77.32   & 68.18   & 3.80E-02  & 2.94E-04 & 400                  & 143.60  & 78.4    & 3.34E-03  & 3.58E-04 \\
		& 20     & 145   & 11    & 400        & 103.57  & 14.47   & 2.94E-02  & 4.52E-04 & 600                  & 189.71  & 29.13   & 2.63E-03  & 4.43E-04 \\
		& 20     & 261   & 21    & 400        & 233.03  & 69.82   & 1.13E-02  & 7.28E-04 & 600                  & 421.62  & 18.64   & 1.01E-03  & 6.32E-04 \\
		& 20     & 378   & 31    & 400        & 309.93  & 289.49  & 6.80E-02  & 3.51E-04 & 800                  & 1583.43  & 1311.51 & 6.62E-03  & 4.37E-04 \\
		& 36     & 264   & 11    & 300        & 389.47  & 329.88  & 3.83E-03  & 1.84E-04 & 1200                 & 5707.40  & 5069.82 & 3.07E-04  & 2.09E-04 
	\end{tblr}
	\label{table:mps_compare}
\end{table*}

==> tables/single.tex <==
\begin{table}[]
	\centering
	\caption{\textsc{1-Qubit Gate}}
	\begin{tabular}{|c|c|c|c|}
		\hline
		H               & $\frac{1}{\sqrt{2}}\begin{pmatrix}
			1 & 1  \\
			1 & -1
		\end{pmatrix}$                     &
		X ($\sigma_x $) & $\begin{pmatrix}
			0 & 1 \\
			1 & 0
		\end{pmatrix}$                                                 \\
		\hline
		Y ($\sigma_y $) & ${\left(\begin{matrix}
				0 & -i \\
				i & 0
			\end{matrix}\right)}$                                 &
		Z ($\sigma_z $) & $\left(\begin{matrix}
			1 & 0  \\
			0 & -1
		\end{matrix}\right)$                                     \\
		\hline
		% S & ${\left(\begin{matrix}
				% 1 & 0 \\
				% 0 & i
				% \end{matrix}\right)}$ &
		T               & ${\left(\begin{matrix}
				1 & 0           \\
				0 & e^{i \pi/4}
			\end{matrix}\right)}$                                 &
		$R_x(\theta)$   & ${\left(\begin{matrix}
				\cos \frac{\theta}{2}    & -i \sin \frac{\theta}{2} \\
				-i \sin \frac{\theta}{2} & \cos \frac{\theta}{2}
			\end{matrix}\right)}$     \\
		\hline
		$R_y(\theta)$   & ${\left(\begin{matrix}
				\cos \frac{\theta}{2} & -\sin \frac{\theta}{2} \\
				\sin \frac{\theta}{2} & \cos \frac{\theta}{2}
			\end{matrix}\right)}$      &
		$R_z(\theta)$   & ${\left(\begin{matrix}
				e^{-i \theta / 2} & 0                \\
				0                 & e^{i \theta / 2}
			\end{matrix}\right)}$                    \\
		\hline
	\end{tabular}
	\label{table:single}
\end{table}
